Model-Based Safety-Cases for Software-Intensive Systems

Safety cases become increasingly important for software certification. Models play a crucial role in building and combining information for the safety case. This position paper sketches an ideal model-based safety case with defect hypotheses and failure characterisations. From this, open research issues are derived.

==> method.tex <==
\section{Method (Peter)}\label{sec:method}

Model-based development is the basis for applying an integrated
approach for constructing both safety cases and systems in a seamless
process. It is our goal to integrate system engineering processes for
embedded systems with known techniques for constructing safety cases.

The following steps are substantial parts of our method. 
\begin{description}
\item[Domain analysis:] As stated above explicit \emph{hypotheses of
    defects} and a \emph{characterisation of failures} is essential.
\item[Requirements analysis:] \emph{Safety requirements} and
  \emph{hazards} have to be identified. Furthermore a risk assessment
  is necessary. 
\item[Model building:] Parallel to the system design, \emph{safety
    relevant information} is added to the model respectively design
  elements.  Furthermore an \emph{environment} and an \emph{operator
    model} is build and explicitly added to the overall model.
\item[Safety analysis:] During the whole system development process
  safety analyses are done. In the early phases they help to
  \emph{refine and clarify requirements} and to guide the design. In
  the later phases they \emph{confirm achieved safety properties}.
\item[Building safety cases by integration of information:] Based on
  the gathered information the safety cases for the overall systems
  could be constructed from the model.
\end{description}

For the construction of a safety case different types of arguments are
needed:
\begin{description}
\item[Quantitative methods] can be further classified into
  \begin{description}
  \item[probabilistic methods] like MTTF, MTTR, ...
  \item[deterministic methods] like formal proofs, exhaustive tests,
  ... 
  \end{description}
\item[Qualitative methods] claim the compliance with some rules or
  standards which are generally accepted like coding, testing or
  developing standards.
\end{description}

Within an integrated approach these different types of arguments
should be compositional -- i.e., during a safety analysis different
methods could be used to compose a line of argument. As both
qualitative and quantitative methods have to be used for an efficient
development of safety cases the composition is a crucial point.
Furthermore for different goals different methods are adequately used.


